Structural features of jammed-granulate metamaterials

Granular media near jamming exhibit fascinating properties, which can be harnessed to create jammed-granulate metamaterials: materials whose characteristics arise not only from the shape and material properties of the particles at the microscale, but also from the geometric features of the packing. For the case of a bending beam made from jammed-granulate metamaterial, we study the impact of the particles' properties on the metamaterial's macroscopic mechanical characteristics. We find that the metamaterial's stiffness emerges from its volume fraction, in turn originating from its creation protocol; its ultimate strength corresponds to yielding of the force network. In contrast to many traditional materials, we find that macroscopic deformation occurs mostly through affine motion within the packing, aided by stress relieve through local plastic events, surprisingly homogeneously spread and persistent throughout bending.

==> media/img/simSetup/beamSketch.tex <==
% tikzpic.tex
% tikzpic.tex
% \documentclass[crop,tikz]{standalone}% 'crop' is the default for v1.0, before it was 'preview'
%\usetikzlibrary{...}% tikz package already loaded by 'tikz' option
% \begin{document}
\begin{tikzpicture}[scale=1,cross/.style={path picture={ 
  \draw[black]
    (path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);
  }}]
  \centering
  % Load
  \draw [-] (2,1) circle (0.2);
  \draw [-] (4,1) circle (0.2);
  \draw[->] (2,1.4) node [left] {$\vec{v}$} -- (2,1.2);
  \draw[->] (4,1.4) node [left] {$\vec{v}$} -- (4,1.2);
  %\draw[->] (4,1) node [above] {$F/2$} -- (4,0.8);

  % Beam
  \draw [-] (-0.1,0) rectangle (6.1,0.8);
  % supports
  \draw [-] (-0.3,-0.3) -- (0,0) -- (0.3,-0.3);
  \draw [-] (6-0.3,-0.3) -- (6,0) -- (6.3,-0.3);

  % Deflected beam
  \draw [-, dotted] (-0.1,0.8) to [out=-15, in=-165](6.1,0.8) {};
  \draw [-, dotted] (-0.1,0) to [out=-15, in=-165](6.1,0) {};
  \draw[<->] (3,0) -- (3,-0.4) node[midway, right]{$\Delta z(L/2)$};

  % X- Axis
  \draw[-] (-0.35,-0.6) -- (0,-0.6);
  \draw[|-|] (0,-0.6) node[below]{$0$} -- (2,-0.6) node[below]{$L/3$};
  \draw[-|] (2,-0.6) -- (4,-0.6) node[below]{$2L/3$};
  \draw[-|] (4,-0.6) -- (6,-0.6) node[below]{$L$};
  \draw[->] (6,-0.6) -- (6.5,-0.6) node[below]{$x$\quad};
  
  % Z - Axis
  \draw[-|] (-0.5,-0.45) -- (-0.5,0) node[left]{$-h/2$};
  \draw[-|] (-0.5,-0) -- (-0.5,0.4) node[left]{$0$};
  \draw[-|] (-0.5,0.4) -- (-0.5,0.8)  node[left]{$h/2$};
  \draw[->] (-0.5,0.8) -- (-0.5,1.3)  node[left]{$z$};

  % Y - Axis
  \node [draw,circle,cross,minimum width=0.04](B) at (-0.5,-0.6){};
  \node at (-0.7,-0.8) {$y$};
  % \node [draw,circle,cross,minimum width=0.06](B) at (-1.0,-0.5){};
  % \node at (-0.8,-0.3) {$y$};
  
\end{tikzpicture}
% \end{document}


==> media/img/simSetup/schematic_procedure.tex <==
\tikzstyle{block} = [draw, rectangle, minimum height=4em, minimum width=8em, text width =8em, align=center]

% The block diagram code is probably more verbose than necessary
\begin{tikzpicture}[auto, node distance=2cm,>=latex', font = \small]
	
    % We start by placing the blocks
    \node [name=input] (input) at (0,0) {};
    \node [block, right =0.0cm of input, darkgray] (seedingtwo) {seeding};
    \node [block, right =0.5cm of seedingtwo, darkgray] (growthtwo) {particle growth\\until $\phi\geq\phi_\text{init}$};
	\node [block, right =0.5cm of growthtwo, darkgray, minimum width=9em, text width =9em] (vacuumtwo) {application of\\confining pressure};
	\node [block, right =0.5cm of vacuumtwo, darkgray, minimum width=9em, text width =10em] (bendingtwo) 
	{bending test\\starting at $\phi_\text{bend}(\mu_\text{init})$};
	
	\node [above = 0.37cm of seedingtwo] (stepone) {step \textsc{i}};
	\node [above = 0.37cm of growthtwo] (steptwo) {step \textsc{ii}};
	\node [above = 0.37cm of vacuumtwo] (stepthree) {step \textsc{iii}};
	\node [above = 0.37cm of bendingtwo] (stepfour) {step \textsc{iv}};
	
	\draw[->, darkgray] (seedingtwo)  -- (growthtwo);
	\draw[->, darkgray] (growthtwo) -- node[midway, name=midpostwo]{} (vacuumtwo);
	\draw[->, darkgray] (vacuumtwo) -- node[midway, name=midpostwotwo]{} (bendingtwo);
	
	\node [above =0.5cm of midpostwo] (pptytwo) {$\mu = \mu_\text{init}$};
	\draw [] (midpostwo.-90) -- (pptytwo);
	\node [above =0.5cm of midpostwotwo] (pptytwo) {$\mu = \mu_\text{p}$};
	\draw [] (midpostwotwo.-90) -- (pptytwo);
\end{tikzpicture}

